Photometric Redshifts Probability Density Estimation from Recurrent Neural Networks in the DECam Local Volume Exploration Survey Data Release 2

Photometric wide-field surveys are imaging the sky in unprecedented detail. These surveys face a significant challenge in efficiently estimating galactic photometric redshifts while accurately quantifying associated uncertainties. In this work, we address this challenge by exploring the estimation of Probability Density Functions (PDFs) for the photometric redshifts of galaxies across a vast area of 17,000 square degrees, encompassing objects with a median 5$\sigma$ point-source depth of $g$ = 24.3, $r$ = 23.9, $i$ = 23.5, and $z$ = 22.8 mag. Our approach uses deep learning, specifically integrating a Recurrent Neural Network architecture with a Mixture Density Network, to leverage magnitudes and colors as input features for constructing photometric redshift PDFs across the whole DECam Local Volume Exploration (DELVE) survey sky footprint. Subsequently, we rigorously evaluate the reliability and robustness of our estimation methodology, gauging its performance against other well-established machine learning methods to ensure the quality of our redshift estimations. Our best results constrain photometric redshifts with the bias of $-0.0013$, a scatter of $0.0293$, and an outlier fraction of $5.1\%$. These point estimates are accompanied by well-calibrated PDFs evaluated using diagnostic tools such as Probability Integral Transform and Odds distribution. We also address the problem of the accessibility of PDFs in terms of disk space storage and the time demand required to generate their corresponding parameters. We present a novel Autoencoder model that reduces the size of PDF parameter arrays to one-sixth of their original length, significantly decreasing the time required for PDF generation to one-eighth of the time needed when generating PDFs directly from the magnitudes.

==> Body/keywords.tex <==
\begin{keywords} % for mnras
galaxies: fundamental parameters \mysep 
galaxies: structure \mysep 
techniques: image processing \mysep
methods: miscellaneous \mysep
surveys
\end{keywords}

==> Body/pdf-compression.tex <==
\section{Compressing Probability Density Functions}


    Having the entire photo-z PDFs for galaxies would be the best scenario once it allow us to apply more robust statistical methods on the results, having a major understanding about cosmological parameters and features.  
    
    Unfortunately, it is unfeasible to store all the PDfs and give easy and free access to them. Our PDFs were generated on 1000 values of redshift between  0 and 1.5 equally spaced. To store 10,000 PDFs with this configuration on a .fits file would be necessary $\approx 80 MBytes$ of space on disk. The area of 17,000$deg^2$ of DELVE DR2 covering $griz$ bands simultaneously, would corresponds to $\approx1,700,000,000$ objects, i.e, the PDFs for all of these objects would need $\approx 12 TBytes$ on disk. 

    We can reduce the space needed since our PDFs are fully defined by $\alpha$'s, $\mu$'s and $\sigma$'s. Storing just the 60 parameters for each object, our estimate of space would be reduced to $\approx 40 GBytes$, which is a considerable improvement. Nevertheless, with the upcoming wide field surveys such as LSST, the number of galaxies observed per night is expected to be around 100,000,000. In that sense we developed a \textit{Autoencoder} model to compact even more our PDFs information.

    The Autoencoder's compose a class of deep learning models that explore the capacity of deep learning to identify, extract and transform features from the input data. This model is comprised of a \textit{encoder} part that reduces the dimensionality of the input, often into 1-D latent vector (element of what we call latent spacer). The other part is the \textit{decoder} that transform a vector from the latent space into the desirable output, which is, in our case, the input itself.
    Autoencoder models are commonly used on image processing tasks, such as simulation [] or image compression.
    %It's clear that have the entire PDFs of redshifts is important because them allow us to make 
    % \subsection{Autoencoders}
    
    \subsection{architecture overview}
                    
        Our autoencoder model does not follow the standard applications of autoencoders, in the sense that it is fully comprised of Dense layers, instead the convolutional ones.
        We can see the archtecure scheme on the Figure \ref{fig:autoencoder_architecture}.
        
        The encoder part of the model is composed of one layer that read the input parameters separately and pass each one of them trough a Dense layer with 16 neurons and a linear activation. Then, all the outputs of the Dense layers are concatenated and pass trough a Dense layer similar the last ones but with a Relu activation. The output of the encoder is a latent vector with size 10, and Linear activation. 

        The decoder part reads the latent vector with three different "paths[?]" independently, each one corresponding to a different PDF parameter set. The $\sigma$-path is composed of two Dense layers, both with nnelu activation, with the first one containing 16 neurons and the second with $C$(number of components) neurons. The nnelu activation functions were chose in order to  avoid $\sigma$'s negative indefinite values, for those Normal distributions are note defined.
        The $\mu$-path is similar to the $\sigma$ one, but with the first and second layers activation being \textit{tanh} and \textit{linear}, respectively. There is no restriction on the means of the Normal distributions that compose the PDF, at principle, so we maintened the linear activation function as output. The tanh function was chose empirically to avoid higher values on the network weights. Several tests with other combinations of activation functions were made, and the tang-linear combination gave the best performance achieved. 
        The $\alpha$-path follows the same, but with Relu and \textit{softmax} as activation on the first and second layers, respectively. The chose of the activation regards the fact that all the alphas have to be positive, less than 1 and sum to a unit.
        % obey $0<\alpha_i<1$ and they have to sum to 1 .  
        
        \begin{figure}
            \centering
            \includegraphics[width=0.8\linewidth]{Figures/Nets/autoencoder_architecture.png}
            \caption{Autoencoder architecture.}
            \label{fig:autoencoder_architecture}
        \end{figure}
    
        

        
    \subsection{Training, validation and testing}
        
        We used the PDFs generated by our MDN model trained with the A dataset to the autoencoder training process, since the photo-z's will be generate by this MDN model. We also maintained the training dataset as beeng the A set. The test data was also the composed of the same objects as the one used to test the MDN model.

        To validate the consistency of the autoencoder model during the train process, we made a cross validation similar to the one made on the MDN process, maintaining the respectives objects for each fold. We can see on Figure \ref{fig:autoencoder_loss} the convergence between the train and validation data for all the folds. We chose the model that corresponded to the smallest loss value of all the folds.

        
        
        \begin{figure}
            \centering
            \includegraphics[width=\linewidth]{Figures/results/autoencoder_loss.png}
            \caption{Training and validation curves for the Autoencoder model. The shaded area corresponds to the errors given by the cross validation process.}
            \label{fig:autoencoder_loss}
        \end{figure}
        
        Following our initial estimates, this technique at the current stage could reduce the first $40Gbytes$ given by the storage of the 60 PDF's components, into $\approx 7GBytes$ of space in disk, that corresponds to the storage of the 10-valued latent vectors.

        
    \subsection{Photo-z statistics recovered }

        {\color{purple} talvez incluir kbl divergence...}
        
        We compared the reconstructed PDFs with the original ones using the pont-like metrics. The results are showed in the Figure \ref{fig:recovered_metrics}. The reconstructed metrics are in agreement with the original within the expected uncertainty given by the cross validation, except for the $\sigma_{NMAD}$. There are two spikes on $\sigma_{NMAD}$ at $z\tilde 0.1$ and $z\tilde 0.2$ that considerably run out of the expected deviation. The causes of these spikes could be related to the autoencoder architecture, what will be discussed in more details at the discussion section. 
        
        % To compare the quality of the reconstructed PDFs with the original ones, we used the point-like metrics

    
        \begin{figure}
            \centering
            \includegraphics[width=\linewidth]{Figures/results/reconstruct_PDF.png}
            \caption{Recovered point-like metrics in contrast to the original metrics for the A training dataset.}
            \label{fig:recovered_metrics}
        \end{figure}

